Fifty Years of MIMO Detection: The Road to Large-Scale MIMOs

The emerging massive/large-scale MIMO (LS-MIMO) systems relying on very large antenna arrays have become a hot topic of wireless communications. Compared to the LTE based 4G mobile communication system that allows for up to 8 antenna elements at the base station (BS), the LS-MIMO system entails an unprecedented number of antennas, say 100 or more, at the BS. The huge leap in the number of BS antennas opens the door to a new research field in communication theory, propagation and electronics, where random matrix theory begins to play a dominant role. In this paper, we provide a recital on the historic heritages and novel challenges facing LS-MIMOs from a detection perspective. Firstly, we highlight the fundamentals of MIMO detection, including the nature of co-channel interference, the generality of the MIMO detection problem, the received signal models of both linear memoryless MIMO channels and dispersive MIMO channels exhibiting memory, as well as the complex-valued versus real-valued MIMO system models. Then, an extensive review of the representative MIMO detection methods conceived during the past 50 years (1965-2015) is presented, and relevant insights as well as lessons are inferred for designing complexity-scalable MIMO detection algorithms that are potentially applicable to LS-MIMO systems. Furthermore, we divide the LS-MIMO systems into two types, and elaborate on the distinct detection strategies suitable for each of them. The type-I LS-MIMO corresponds to the case where the number of active users is much smaller than the number of BS antennas, which is currently the mainstream definition of LS-MIMO. The type-II LS-MIMO corresponds to the case where the number of active users is comparable to the number of BS antennas. Finally, we discuss the applicability of existing MIMO detection algorithms in LS-MIMO systems, and review some of the recent advances in LS-MIMO detection.

==> figtex2pdf <==
#!/bin/bash
#
# Wrapper for figtex2eps so that it can produce
# pdf output.
# 
# Basically runs figtex2eps on the same fig file, but
# then applies epstopdf to the result.
#
# $Id: figtex2pdf,v 1.3 2003/10/28 18:55:32 berland Exp $
#

function die
{
    echo "$1"
    echo "Exiting..."
    exit
}

# Check if gptex2eps exists in $PATH
which figtex2eps >/dev/null 2>&1 \
    || die " (Error) Could not find 'figtex2eps'. It must be installed for figtex2pdf to work."

figtex2eps -pdf "$@"

==> makeglossaries <==
#!/usr/bin/env perl

# File    : makeglossaries
# Author  : Nicola Talbot
# Version : 2.03 (2011/12/02)
# Description: simple Perl script that calls makeindex or xindy.
# Intended for use with "glossaries.sty" (saves having to remember
# all the various switches)

# This file is distributed as part of the glossaries LaTeX package.
# Copyright 2007 Nicola L.C. Talbot
# This work may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.3
# of this license or any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.3 or later is part of all distributions of LaTeX
# version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
#
# The Current Maintainer of this work is Nicola Talbot.

# This work consists of the files glossaries.dtx and glossaries.ins 
# and the derived files glossaries.sty, mfirstuc.sty,
# glossary-hypernav.sty, glossary-list.sty, glossary-long.sty,
# glossary-super.sty, glossaries.perl.
# Also makeglossaries and makeglossaries.

my $version="2.03 (2011-12-02)";

# History:
# v2.03 (2011-04-12):
#   * added warning about possibly needing 'nomain' package option
# v2.02 (2011-04-2):
#   * Prints version number at start of run unless -q
#   * Added more diagnostics.
# v2.01 (2010-09-29):
#   * Added 'use warnings'
# v2.0 (2010-06-30) :
#   * Made file handle local in &scan_aux
# v1.9 (2010-06-14) :
#   * Check for \@input
# v1.8 (2009-11-03) :
#   * Create an empty output file if the input file is empty
#     without calling xindy/makeindex
# v1.7 (2009-09-23) :
#   * Issue warning rather than error when empty/non existant file 
#     checks fail
# v1.6 (2009-05-24) :
#   * main glossary no longer automatically added
#     (only added if information in aux file)
#   * if file extension is specified, check added to ensure it
#     corresponds to a known glossary extension.
#   * added file existance test and file empty test
# v1.5 (2008-12-26) :
#   * added support for xindy
#   * picks up ordering information from aux file
# v1.4 (2008-05-10) :
#   * added support for filenames with spaces.
# v1.3 (2008-03-08) :
#   * changed first line from /usr/bin/perl -w to /usr/bin/env perl
#     (Thanks to Karl Berry for suggesting this.)
# v1.2 (2008-03-02) :
#   * added support for --help and --version
#   * improved error handling
# v1.1 (2008-02-13) :
#   * added -w and strict
#   * added check to ensure .tex file not passed to makeglossaries
#
# v1.0 (2007-05-10) : Initial release.

use Getopt::Std;
use strict;
# v2.01 added the following line
use warnings;
use vars qw($opt_q $opt_t $opt_o $opt_s $opt_p $opt_g $opt_c $opt_r
   $opt_l $opt_i $opt_L $opt_n $opt_C);


$Getopt::Std::STANDARD_HELP_VERSION = 1;

# v1.5 added -L <lang> for xindy (but language can be specified in 
# .tex file)
# v1.5 added -n (print the command that would be issued but
# don't actually run the command)
getopts('s:o:t:p:L:C:ilqrcgn');

unless ($#ARGV == 0)
{
   die "makeglossaries: Need exactly one file argument.\n",
       "Use `makeglossaries --help' for help.\n";
}

# v2.02: added:
print "makeglossaries version $version\n" unless ($opt_q);

# v2.02: added:
my $xdynotist = 1;
my $needcompatibilitymode=2;

# define known extensions

# v1.6: removed adding main glossary here as there's no guarantee
# that it's been used. If it has been used, the information will
# be picked up later in the aux file
my %exttype = (
#   main => {in=>'glo', out=>'gls', 'log'=>'glg'},
 );

# v1.5 define require languages for xindy

my %language = ();
my %codepage = ();

my $ext = '';
my $name = $ARGV[0];

# modified this to make sure users don't try passing the
# tex file:
if (length($ARGV[0]) > 3 and substr($ARGV[0],-4,1) eq ".")
{
  $name = substr($ARGV[0],0,length($ARGV[0])-4);

  $ext = substr($ARGV[0],-3,3);

  if (lc($ext) eq 'tex')
  {
     die("Don't pass the tex file to makeglossaries:\n"
        ."either omit the extension to make all the glossaries, "
        ."or specify one of the glossary files, e.g. $name.glo, to "
        ."make just that glossary.\n")
  }
}

# v2.01 add check to see if aux file exists

unless (-e "$name.aux")
{
   die "Auxiliary file '$name.aux' doesn't exist. Have you run LaTeX?\n";
}

my $istfile = "";

# should letter ordering be used? (v1.5 added)

my $letterordering = defined($opt_l);

# check aux file for other glossary types
# and for ist file name

&scan_aux($name);

# has the style file been specified?
unless ($istfile)
{
   die "No \\\@istfilename found in '$name.aux'.\n",
       "Did your LaTeX run fail?\n",
       "Did your LaTeX run produce any output?\n",
       "Did you remember to use \\makeglossaries?\n";
}

# v1.5 save the general xindy switches

my $xdyopts = '';

# v2.01 replaced 'unless ($opt_L eq "")' with 'if ($opt_L)'
if ($opt_L)
{
  $xdyopts .= " -L $opt_L";
}

# save all the general makeindex switches

my $mkidxopts = '';

if ($opt_i)
{
   $mkidxopts .= " -i";
}

if ($letterordering)
{
   $mkidxopts .= " -l";
   $xdyopts .= " -M ord/letorder";
}

if ($opt_q)
{
# v2.01 removed following lines. (This script now deals with
# printing messages to STDOUT.)
   #$mkidxopts .= " -q";
   #$xdyopts .= " -q";
}

if ($opt_r)
{
   $mkidxopts .= " -r";
}

if ($opt_c)
{
   $mkidxopts .= " -c";
}

if ($opt_g)
{
   $mkidxopts .= " -g";
}

# v2.01 replaced 'unless ($opt_p eq "")' with 'if ($opt_p)'
if ($opt_p)
{
   $mkidxopts .= " -p $opt_p";
}

# v2.01 replaced 'unless ($opt_s eq "")' with 'if ($opt_s)'
if ($opt_s)
{
   # v2.01 check if user has specified -s <file>.ist but aux file
   # indicates .xdy ought to be used and vice-versa. Also check if
   # requested style file exists

   unless (-e $opt_s)
   {
      die "\n",
         "Requested style file '$opt_s' doesn't exist.\n\n";
   }

   if ($istfile=~/\.xdy$/ and $opt_s!~/\.xdy$/)
   {
      die "\n",
        "The auxiliary file indicates that you should be using xindy,\n",
        "but you have specified makeindex style file '$opt_s'\n",
        "Make sure you don't specify 'xindy' as a package option if\n",
        "you want to use makeindex.\n\n",
        "\\usepackage[makeindex]{glossaries}\n\n";
   }
   elsif ($istfile!~/\.xdy$/ and $opt_s=~/\.xdy$/)
   {
      die "\n",
        "The auxiliary file indicates that you should be using\n",
        "makeindex, but you have specified xindy style file '$opt_s'.\n",
        "Make sure you specify 'xindy' as a package option if you\n",
        "want to use xindy.\n\n",
        "\\usepackage[xindy]{glossaries}\n\n";
   }

   $istfile = $opt_s;
}

# Use xindy if style file ends with .xdy otherwise use makeindex

my $usexindy = ($istfile=~m/\.xdy\Z/);

if ($ext)
{
   # an extension has been specified, so only process
   # the specified file

   # v1.6 %thistype is no longer given a default value
   my %thistype;

   my $thislang = "";
   my $thiscodepage = "";

   foreach my $type (keys %exttype)
   {
      if ($exttype{$type}{'in'} eq $ext)
      {
         %thistype = %{$exttype{$type}};

         $thislang = $language{$type};

         $thiscodepage = $codepage{$type};

         last;
      }
   }

   # v1.6 If %thistype hasn't been defined, then the given
   # extension doesn't correspond to any known glossary type

   # v2.01 replaced deprecated 'defined(%thistype)' with %thistype
   unless (%thistype)
   {
      die "The file extension '$ext' doesn't correspond to any\n",
          "known glossary extension. Try running makeglossaries\n",
          "without an extension, e.g. makeglossaries \"$name\".\n";
   }

   my $outfile;

# v2.01 replaced 'if ($opt_o eq "")' with 'unless ($opt_o)'
   unless ($opt_o)
   {
      $outfile = "$name.$thistype{out}";
   }
   else
   {
      $outfile = $opt_o;
   }

   my $transcript;

# v2.01 replaced 'if ($opt_t eq "")' with 'unless ($opt_t)'
   unless ($opt_t)
   {
      $transcript = "$name.$thistype{'log'}";
   }
   else
   {
      $transcript = $opt_t;
   }

# v2.01 remove old transcript file

   unless ($opt_n)
   {
      unlink($transcript);
   }

   if ($usexindy)
   {
      &xindy("$name.$ext", $outfile, $transcript,$istfile,
        $thislang, $thiscodepage, $xdyopts, $opt_q, $opt_n);
   }
   else
   {
      &makeindex("$name.$ext",$outfile,$transcript,$istfile,
                 $mkidxopts,$opt_q, $opt_n);
   }
}
else
{
   # no file extension specified so process all glossary types

   foreach my $type (keys %exttype)
   {
      my %thistype = %{$exttype{$type}};

      my $inputfile = "$name.$thistype{in}";

      my $outfile;

# v2.01 changed 'if ($opt_o eq "")' with 'unless ($opt_o)'
      unless ($opt_o)
      {
         $outfile = "$name.$thistype{out}";
      }
      else
      {
         $outfile = $opt_o;
      }

      # v1.7 print warnings to STDOUT instead of STDERR

      # v1.6 added file existance test
      unless (-e $inputfile)
      {
         print "Warning: File '$inputfile' doesn't exist.\n",
             "*** Skipping glossary '$type'. ***\n";
         next;
      }

      unless (-r $inputfile)
      {
         print "Warning: No read access for '$inputfile' $!\n",
             "*** Skipping glossary '$type'. ***\n";
         next;
      }

      my $transcript;

# v2.01 changed 'if ($opt_t eq "")' with 'unless ($opt)'
      unless ($opt_t)
      {
         $transcript = "$name.$thistype{'log'}";
      }
      else
      {
        $transcript = $opt_t;
      }

      # v1.6 added file empty test
      if (-z $inputfile)
      {
         my $message =
             "Warning: File '$inputfile' is empty.\n".
             "Have you used any entries defined in glossary '$type'?\n";

         if ($type eq 'main')
         {
            $message .=
               "Remember to use package option 'nomain' if you\n".
               "don't want to use the main glossary.\n";
         }

         warn $message;

         # Write warning to transcript file.

         if (open TRANSFD, ">$transcript")
         {
            print TRANSFD $message;
            close TRANSFD;
         }

         # create an empty output file and move on to the next glossary

         if (open OFD, ">$outfile")
         {
            print OFD "\\null\n";
            close OFD;
         }
         else
         {
            print STDERR "Unable to create '$outfile' $!\n";
         }

         next;
      }

# v2.01 remove old transcript file

      unless ($opt_n)
      {
         unlink($transcript);
      }

      if ($usexindy)
      {
         &xindy($inputfile,$outfile,$transcript,$istfile,
                $language{$type},$codepage{$type},
                $xdyopts,$opt_q,$opt_n);
      }
      else
      {
         &makeindex($inputfile,$outfile,$transcript,
                    $istfile,$mkidxopts,$opt_q,$opt_n);
      }
   }
}

sub scan_aux{
  my $name = shift;

  # v2.0 added
  local(*AUXFILE);

  if (open AUXFILE, "$name.aux")
  {
     while (<AUXFILE>)
     {
        # v1.9 added
        if (m/\\\@input{(.+)\.aux}/)
        {
           &scan_aux($1);
        }

        if (m/\\\@newglossary\s*\{(.*)\}{(.*)}{(.*)}{(.*)}/)
        {
           $exttype{$1}{'log'} = $2;
           $exttype{$1}{'out'} = $3;
           $exttype{$1}{'in'}  = $4;

           unless ($opt_q)
           {
              print "added glossary type '$1' ($2,$3,$4)\n";
           }
        }

        if (m/\\\@istfilename\s*{([^}]*)}/)
        {
           $istfile = $1;

           # check if double quotes were added to \jobname
           $istfile=~s/^"(.*)"\.ist$/$1.ist/;
        }

        # v1.5 added
        if (m/\\\@xdylanguage\s*{([^}]+)}{([^}]*)}/)
        {
           $language{$1} = $2;
        }

        # v1.5 added
        if (m/\\\@gls\@codepage\s*{([^}]+)}{([^}]*)}/)
        {
           $codepage{$1} = $2;
        }

        # v1.5 added
        # Allow -l switch to override specification in aux file
        unless (defined($opt_l))
        {
           if (m/\\\@glsorder\s*{([^}]+)}/)
           {
              my $ordering = $1;

              if ($ordering eq "word")
              {
                 $letterordering = 0;
              }
              elsif ($ordering eq "letter")
              {
                 $letterordering = 1;
              }
              else
              {
                 print STDERR
                   "Unknown ordering '$ordering'\n",
                   "Assuming word ordering\n";
                 $letterordering = 0;
              }
           }
        }
     }

     close AUXFILE;
  }
  else
  {
     print STDERR "Unable to open $name.aux: $!\n";
  }
}

# v2.01 new subroutine run_app added
sub run_app{
   my($appname, $appargs, $trans, $quiet, $dontexec) = @_;

   local(*STATUS);

   my $status   = '';
   my $warnings = '';
   my $errno = 0;
   my $log = '';

   print "$appname $appargs\n" if ($dontexec or not $quiet);

   return if ($dontexec);

   if (open (STATUS, "$appname $appargs 2>&1 |"))
   {
      while (<STATUS>)
      {
         print unless ($quiet);

         $warnings .= $_ if (/WARNING:/);

         $status .= $_ unless (/^[\w]+ing/ or /^Finished/ or /^Usage:/);

         $log .= $_;
      }

      close STATUS;
   }
   else
   {
      $warnings = "WARNING: Unable to fork $appname: $!\n";

      print STDERR $warnings, "Retrying without redirection.\n";

      $status = `$appname $appargs`;

      $log = $status;

      print $status unless ($quiet);
   }

   if ($?)
   {
      $errno = $?;

      if (open LOGFILE, ">>$trans")
      {
         print LOGFILE "\n\n*** Unable to execute: '$appname $appargs' ***\n\n";
         print LOGFILE "Status report:\n\n";
         print LOGFILE "$log";
         close LOGFILE;
      }
      else
      {
         print STDERR "Unable to open '$trans' $!\n";
      }
   }

   if ($log=~/\(0 entries accepted,/)
   {
      # Attempt to diagnose what's gone wrong

      if (open TRANS, $trans)
      {
         while (<TRANS>)
         {
            if (/Unknown specifier ;/)
            {
               $errno = $xdynotist;

               last;
            }
         }

         close TRANS;
      }

   }

   return ($status, $warnings, $errno);
}

sub makeindex{
   my($in,$out,$trans,$ist,$rest,$quiet,$dontexec) = @_;

   my $args = "$rest -s \"$ist\" -t \"$trans\" -o \"$out\" \"$in\"";

# v2.01 replaced code with call to &run_app

   my ($status, $warnings, $errno) 
     = &run_app('makeindex', $args, $trans, $quiet, $dontexec);

   return if ($dontexec);

   if ($errno)
   {
      my $diagnostic = '';

      if ($errno = $xdynotist)
      {
         $diagnostic =
           "Style name indicates makeindex, but may be in xindy format.\n"
          . "Remember to use \\setStyleFile to specify the name\n"
          . "of the style file rather than redefining \\istfilename\n"
          . "explicitly.";
      }

      die "\n***Call to makeindex failed***\n", 
        ($diagnostic ?
          "\nPossible cause of problem:\n\n".  $diagnostic . "\n\n":
          "\n"
        ),
        "Check '$trans' for details\n";
   }
}

sub xindy{
   my($in,$out,$trans,$ist,$language,$codepage,$rest,$quiet,
     $dontexec) = @_;
   my($args, $langparam, $main, $retry);
   my($module);

   $module = $ist;
   $module=~s/\.xdy\Z//;

   unless (defined($language))
   {
      $language = '';
   }

   # map babel names to xindy names
   if ($language eq "frenchb")
   {
      $language = "french";
   }
   elsif ($language=~/^n?germanb?$/)
   {
      $language = "german";
   }
   elsif ($language eq "magyar")
   {
      $language = "hungarian";
   }
   elsif ($language eq "lsorbian")
   {
      $language = "lower-sorbian";
   }
   elsif ($language eq "norsk")
   {
      $language = "norwegian";
   }
   elsif ($language eq "portuges")
   {
      $language = "portuguese";
   }
   elsif ($language eq "russianb")
   {
      $language = "russian";
   }
   elsif ($language eq "slovene")
   {
      $language = "slovenian";
   }
   elsif ($language eq "ukraineb")
   {
      $language = "ukrainian";
   }
   elsif ($language eq "usorbian")
   {
      $language = "upper-sorbian";
   }

   if ($language)
   {
     $langparam = "-L $language";
   }
   else
   {
     $langparam = "";
   }

   # most languages work with xindy's default codepage, but
   # some don't, so if the codepage isn't specific, check
   # the known cases that will generate an error
   # and supply a default. (For all other cases, it's up to the 
   # user to supply a codepage.)

# v2.01 changed 'if ($codepage eq "")' to 'unless ($codepage)'
   unless ($codepage)
   {
      if ($language eq 'dutch')
      {
         $codepage = "ij-as-ij";
      }
      elsif ($language eq 'german')
      {
         $codepage = "din";
      }
      elsif ($language eq 'gypsy')
      {
         $codepage = "northrussian";
      }
      elsif ($language eq 'hausa')
      {
         $codepage = "utf";
      }
      elsif ($language eq 'klingon')
      {
         $codepage = "utf";
      }
      elsif ($language eq 'latin')
      {
         $codepage = "utf";
      }
      elsif ($language eq 'mongolian')
      {
         $codepage = "cyrillic";
      }
      elsif ($language eq 'slovak')
      {
         $codepage = "small";
      }
      elsif ($language eq 'spanish')
      {
         $codepage = "modern";
      }
      elsif ($language eq 'vietnamese')
      {
         $codepage = "utf";
      }
   }

   my $codepageparam = "";

   if ($codepage)
   {
      $codepageparam = "-C $codepage";
   }

   $main = join(' ',
      "-I xindy",
      "-M \"$module\"",
      "-t \"$trans\"",
      "-o \"$out\"",
      "\"$in\"");

   $args = join(' ', $rest, $langparam, $codepageparam, $main);

# v2.01 replaced code with call to &run_app

   my ($status, $warnings, $errno) 
     = &run_app('xindy', $args, $trans, $quiet, $dontexec);

   return if ($dontexec);

   if ($status=~/Cannot locate xindy module for language ([^\s]+) in codepage ([^\s]+)/)
   {
      $args = join(' ', $rest, $langparam, $main);

      unless ($quiet)
      {
         my $message = "$&\nRetrying using default codepage.\n";

         print STDERR $message;

         $retry .= $message;
      }

      ($status, $warnings, $errno) 
         = &run_app('xindy', $args, $trans, $quiet, $dontexec);

   }

   if ($status=~/Cannot locate xindy module for language ([^\s]+)/
    and $1 ne 'general')
   {
      $args = join(' ', $rest, "-L general", $main);

      unless ($quiet)
      {
         my $message = "$&\nRetrying with -L general\n";

         print STDERR $message;
         $retry .= $message;
      }

      ($status, $warnings, $errno) 
         = &run_app('xindy', $args, $trans, $quiet, $dontexec);

   }

   if ($errno)
   {
      # attempt further diagnostic

      my $diagnostic = '';

      if ($status=~/index 0 should be less than the length of the string/m)
      {
         $diagnostic = 
           "Sort key required for entries only containing command names";
      }
      elsif ($status=~/variable % has no value/m)
      {
         $diagnostic =
            "Style name has xdy extension, but may be in makeindex format.\n"
          . "Remember to use \\setStyleFile to specify the name\n"
          . "of the style file rather than redefining \\istfilename\n"
          . "explicitly.";
      }
      elsif ($status=~/Possible read-error due to ill-formed string " :sep/m)
      {
         $diagnostic = 
            "You may have missed a \" character in a command such as \\GlsAddXdyLocation";
      }
      elsif (not $language)
      {
         # If the language hasn't been set, then it may be
         # because the document doesn't contain
         # \printglossaries/\printglossary or it may be
         # because the user has a customized style file that
         # contains the language settings.

          $diagnostic = 
          "No language detected.".
          "\nHave you remembered to use \\printglossary\n".
          "or \\printglossaries in your document?";

          if ($in eq 'glo')
          {
             # or it may be that the user doesn't want to use the main
             # glossary and has forgotten to suppress it with the
             # "nomain" package option

             $diagnostic .= 
             "\nRemember to use package option 'nomain' if you don't\n".
             "want to use the main glossary.";
          }
      }

      die "\n***Call to xindy failed***\n", 
          ($diagnostic ? 
          "\nPossible cause of problem:\n\n".  $diagnostic . "\n\n":
          "\n"),
          "Check '$trans' for details\n";
   }

   # Check xindy warnings

   if ($status=~/^WARNING:/m)
   {
      my $diagwarn = '';

      if ($status=~/did not match any location-class/m)
      {
         $diagwarn = "You may have forgotten to add a location \n"
                   . "class with \\GlsAddLocation or you may have \n"
                   . "the format incorrect.\n";

      }

      if ($status=~/unknown attribute `pageglsnumberformat'/m)
      {
         $diagwarn .= "You may need to add 'compatible-2.07' package "
                   .  "option.\n";
      }

      if ($diagwarn)
      {
         warn "\n**Warning:**\n\n", $diagwarn, "\n";

         $warnings .= "\nmakeglossaries diagnostic messages:\n\n"
                   . $diagwarn;
      }
   }

   if ($retry or $warnings)
   {
      if (open LOGFILE, ">>$trans")
      {
         print LOGFILE "\n$warnings";

         if ($retry)
         {
            print LOGFILE "\nmakeglossaries messages:\n\n", $retry;
         }

         close LOGFILE;
      }
      else
      {
         print STDERR "Unable to open '$trans' $!\n";
      }
   }
}

sub HELP_MESSAGE{
   print "\nSyntax : makeglossaries [options] <filename>\n\n";
   print "For use with the glossaries package to pass relevant\n";
   print "files to makeindex or xindy\n\n";
   print "<filename>\tBase name of glossary file(s). This should\n";
   print "\t\tbe the name of your main LaTeX document without any\n";
   print "\t\textension.\n";
   print "\n General Options:\n";
   print "-o <gls>\tUse <gls> as the output file.\n";
   print "-q\t\tQuiet mode\n";
   print "-s <sty>\tEmploy <sty> as the style file\n";
   print "-t <log>\tEmploy <log> as the transcript file\n";
   print "-n\tPrint the command that would normally be executed,\n",
         "\tbut don't execute it\n";

   print "\n Xindy Options:\n";
   print "-L <language>\tUse <language>.\n";

   print "\n Makeindex Options:\n";
   print "-c\t\tCompress intermediate blanks\n";
   print "-g\t\tEmploy German word ordering\n";
   print "-l\t\tLetter ordering\n";   
   print "-p <num>\tSet the starting page number to be <num>\n";
   print "-r\t\tDisable implicit page range formation\n";
   print "\nSee makeindex documentation for further details on these ";
   print "options\n";
}

sub VERSION_MESSAGE{
   print "Makeglossaries Version $version\n";
   print "Copyright (C) 2007 Nicola L C Talbot\n";
   print "This material is subject to the LaTeX Project Public License.\n";
}

1;

=head1 NAME

makeglossaries  - Calls makeindex/xindy for LaTeX documents using glossaries package

=head1 SYNOPSIS

B<makeglossaries> [B<-o> I<file>] [B<-q>] [B<-s> I<file>]
[B<-t> I<file>] [B<-L> I<language>] [B<-c>] [B<-g>] [B<-l>]
[B<-p> I<num>] [B<-r>] [B<--version>] [B<--help>] I<filename>

=head1 DESCRIPTION

B<makeglossaries> is designed for use with LaTeX documents that
use the glossaries package. The mandatory argument I<filename> should
be the name of the LaTeX document without the .tex extension. 
B<makeglossaries> will read the auxiliary file to determine whether
B<makeindex> or B<xindy> should be called. All the information
required to be passed to the relevant indexing application should
also be contained in the auxiliary file, but may be overridden by
the option arguments to B<makeglossaries>.

=head1 OPTIONS

=over 4

=item B<-q>

Quiet mode. Reduces chatter to standard output.

=item B<-o> I<file>

Use I<file> as the output file. (Only suitable for documents 
containing a single glossary, otherwise each glossary will be
overridden.)

=item B<-s> I<file>

Use I<file> as the style file. Note that if you use this option,
you need to know whether B<makeindex> or B<xindy> will be called, as
they have different style files.

=item B<-t> I<file>

Use I<file> as the transcript file.

=item B<-L> I<language>

This option only has an effect if B<xindy> is called. Sets the
language. See B<xindy> documentation for further details.

=item B<-c>

Compress intermediate blanks (B<makeindex> only).

=item B<-g>

Employ German word ordering (B<makeindex> only).

=item B<-l>

Letter ordering (B<makeindex> only).

=item B<-p> I<num>

Sets the starting page number to be I<num> (B<makeindex> only).

=item B<-r>

Disable implicit page range formation (B<makeindex> only).

=item B<--version>

Prints version number and exits.

=item B<--help>

Prints help message and exits.

=back

=head1 REQUIRES

Perl, Getopt::Std, and makeindex or xindy (depending on glossaries
package options).

=head1 LICENSE

This is free software distributed under the LaTeX Project Public 
License. There is NO WARRANTY.
See L<http://www.latex-project.org/lppl.txt> for details.

=head1 AUTHOR

Nicola L. C. Talbot,
L<http://theoval.cmp.uea.ac.uk/~nlct/>

=head1 RECOMMENDED READING

The glossaries manual:

	texdoc glossaries

=cut

